Multiview Equivariance Improves 3D Correspondence Understanding with Minimal Feature Finetuning

Vision foundation models, particularly the ViT family, have revolutionized image understanding by providing rich semantic features. However, despite their success in 2D comprehension, their abilities on grasping 3D spatial relationships are still unclear. In this work, we evaluate and enhance the 3D awareness of ViT-based models. We begin by systematically assessing their ability to learn 3D equivariant features, specifically examining the consistency of semantic embeddings across different viewpoints. Our findings indicate that improved 3D equivariance leads to better performance on various downstream tasks, including pose estimation, tracking, and semantic transfer. Building on this insight, we propose a simple yet effective finetuning strategy based on 3D correspondences, which significantly enhances the 3D correspondence understanding of existing vision models. Remarkably, finetuning on a single object for one iteration results in substantial gains. Our code is available at https://github.com/qq456cvb/3DCorrEnhance.

==> tables/revisitop.tex <==
\begin{table}[t]
    \begin{center}
        \begin{tabular}{lcccc}
        \toprule
        \multirow{2}{*}{Model} & \multicolumn{4}{c}{RevisitOP}\\
        \cmidrule(lr){2-5}
             & Oxford-M & Oxford-H & Paris-M & Paris-H \\
        \midrule
        DINOv2 &  &  &  &  \\
        \quad CLS & 65.16 & 43.26 & 88.85 & 75.92 \\
        \quad CLS + Patch tokens (1 layer)  & 62.35 & 39.00 & 87.69 & 73.69\\
        \quad CLS + Patch tokens (4 layers)  & 48.75 & 19.67 & 79.79 & 60.72\\
        \quad CLS + Patch token (12 layers)  & 26.71 & 6.29 & 54.46 & 26.92\\
        \midrule
        Finetuned  &  &  &  & \\
        \quad CLS & 64.00 & 40.48 & 89.02 & 76.23\\
        \quad CLS + Patch tokens (1 layer)  & 63.45 & 40.04 & 88.62 & 75.43\\
        \quad CLS + Patch tokens (4 layers)  & 51.75 & 22.99 &  81.64 & 63.21\\
        \quad CLS + Patch token (12 layers)  & 35.08 & 9.26 & 64.40 & 36.88\\
        \bottomrule
        \end{tabular}
    \end{center}
    \caption{\textbf{Evaluation of Instance Retrieval on RevisitOP.}}
    \label{tab:revisitop}
\end{table}

